Scale Calibrated Training: Improving Generalization of Deep Networks via Scale-Specific Normalization

Standard convolutional neural networks(CNNs) require consistent image resolutions in both training and testing phase. However, in practice, testing with smaller image sizes is necessary for fast inference. We show that trivially evaluating low-resolution images on networks trained with high-resolution images results in a catastrophic accuracy drop in standard CNN architectures. We propose a novel training regime called Scale calibrated Training(SCT) which allows networks to learn from various scales of input simultaneously. By taking advantages of SCT, single network can provide decent accuracy at test time in response to multiple test scales. In our analysis, we surprisingly find that vanilla batch normalization can lead to sub-optimal performance in SCT. Therefore, a novel normalization scheme called Scale-Specific Batch Normalization is equipped to SCT in replacement of batch normalization. Experiment results show that SCT improves accuracy of single Resnet-50 on ImageNet by 1.7% and 11.5% accuracy when testing on image sizes of 224 and 128 respectively.

==> training.tex <==
\section{Spatial Variant Training}

\begin{figure*}[htb]

\centering
%\vspace*{-0.15in}
\includegraphics[scale=0.2]{latex/figures/pipeline.jpeg}
%\vspace*{-0.1in}

\label{fig: pipeline}
\caption{The overall pipeline: the figure above shows the training step. During the partition phase, fix-sized input images are partitioned to several partitions with different spatial sizes. Then, each partition is forwarded through a convolutional neural network. Since output sizes are different for different partitions, the alignment layer pools them to a common sized so that they can be fed into a fully connected classifier.}
\end{figure*}

In this section, we demonstrate the process of \textit{Spatial Variant Training(SVT)}. The process has three core phases: partition phase, forward phase, and alignment phase. The entire pipeline is demonstrated in Figure 2.
\bigskip\\
\textbf{Partition Phase}. In this phase, a batch of raw images is first passed through standard augmentation procedure, which is usually composed by several augmentation operations followed by a normalization procedure. Then, the transformed batch data $B$ is then converted to $n$ partitions $p_1, p_2, ..., p_n$ according to pre-determined scales $s_1, s_2, ..., s_n$. Each partition $p_i$ contains images with the specific scale corresponding to $s_i$, which is obtained by bilinear interpolation of batch data$B$. 
\bigskip\\
\textbf{Forward Phase}. All partitions $p_1, p_2, ..., p_n$ are forwarded to the convolutional neural network consecutively. The corresponding output feature maps of partitions are then collected before passing through the fully connected classifier. 
\bigskip\\
\textbf{Alignment Phase}. In regular training procedure, it is a common practice to unroll the final output feature map of size $(N, C, H, W)$ to a batch of C-dimensional vectors through max-pooling. In SVT, the final feature maps are of shape $(N, C, H_1, W_1), (N, C, H_2, W_2), ... , (N, C, H_n, W_n)$. In alignment phase, all these feature maps are pooled to batches of C-dimensional vectors adaptively based on their spatial size so that they can be presented to the final fully connected classifier. 
\bigskip\\
\textbf{Testing Phase}. Notice that SVT does not introduce any extra cost in testing. For each batch of testing images, it is directly passed to the forwarding phase. The output of convolutional layers is then directly feed into the fully connected classifier for classification results. 

\begin{figure}[H]
\centering
\vspace*{0.15in}
\includegraphics[scale=0.25]{latex/figures/distribution.png}
%\vspace*{-0.1in}
\caption{Distribution of feature maps outputed by ResNet-32 with BN and Fixup initialization respectively}
\label{fig-stat}
\end{figure}
